Penalising model component complexity: A principled, practical approach to constructing priors

In this paper, we introduce a new concept for constructing prior distributions. We exploit the natural nested structure inherent to many model components, which defines the model component to be a flexible extension of a base model. Proper priors are defined to penalise the complexity induced by deviating from the simpler base model and are formulated after the input of a user-defined scaling parameter for that model component, both in the univariate and the multivariate case. These priors are invariant to reparameterisations, have a natural connection to Jeffreys' priors, are designed to support Occam's razor and seem to have excellent robustness properties, all which are highly desirable and allow us to use this approach to define default prior distributions. Through examples and theoretical results, we demonstrate the appropriateness of this approach and how it can be applied in various situations.

==> Makefile <==
TARGETS = report_short.pdf
DEPS_DIR = .deps
LATEXMK = latexmk -recorder -use-make -deps \
	-e 'warn qq(In Makefile, turn off custom dependencies\n);' \
	-e '@cus_dep_list = ();' \
	-e 'show_cus_dep();'
all : $(TARGETS)

$(foreach file,$(TARGETS),$(eval -include $(DEPS_DIR)/$(file)P))

$(DEPS_DIR) :
	mkdir $@

%.pdf : %.tex
	if [ ! -e $(DEPS_DIR) ]; then mkdir $(DEPS_DIR); fi
	$(LATEXMK) -pdf -dvi- -ps- -deps-out=$(DEPS_DIR)/$@P $<

%.png : %.pdf
	convert $< $@ 

clean :; latexmk -CA

.PHONY: clean


==> proofs2a.tex <==
\section{\PCP s for time-series models}
\subsection{The \PCP\  for the lag-one correlation in an AR(1)
    model}\label{appendix:ar1}

Depending on the application, we will use either $\rho= 0$ (no
dependence in time) or $\rho = 1$ (no changes in time) as the
base model. We assume the AR(1) model has unit marginal precision.
Consider first the case where $\rho=0$ represents the base model and
let $p$ be the dimension. In this case $\mm{\Sigma}_0 = \mm{I}$,
$\mm{\Sigma}_1 = \left(\rho^{|i-j|}\right)$, and then it follows that
$2\text{KLD}(\rho) = (1- p)\log(1-\rho^2)$  
and $d(\rho) =
\sqrt{2\text{KLD}(\rho)}$. With an exponential prior for $d(\rho)$
with rate $\lambda = \theta/\sqrt{p-1}$, we get
\begin{displaymath}
    \pi(\rho) = \frac{\theta}{2} \exp\left(-\theta \sqrt{-\ln(1-\rho^{2})}\right) 
    \; \frac{|\rho|}{(1-\rho^2) \sqrt{-\ln(1-\rho^2)}}, \qquad |\rho|<1.
\end{displaymath}  
To infer $\theta$ we request $(U, \alpha)$ saying that large absolute
correlation are less likely $\Prob(|\rho| > U ) = \alpha$.
This gives $\theta = -\ln(\alpha)/\sqrt{-\ln(1-U^{2})}$.

For the case where $\rho=1$ is the base model, we need to do a
limiting argument, as the base model is singular. Let $\mm{\Sigma}_1 =
\left(\rho^{|i-j|}\right)$ and $\mm{\Sigma}_0 =
\left(\rho_0^{|i-j|}\right)$ where $\rho_0$ is close to $1$ and $\rho
< \rho_0$. We then find that $d(\rho) = C\sqrt{1-\rho}$ for some
constant $C$ not depending on $\rho$.  For simplicity we take $C=1$.
Since $0\le d(\rho) \le\sqrt{2}$, we take a truncated exponential
distribution for $d(\rho)$ with rate $\theta$ and we get
\begin{displaymath}
    \pi(\rho) = \frac{\theta \exp\left(-\theta\sqrt{1-\rho}\right)}{%%
        \left(1-\exp\left(-\sqrt{2}\theta\right)\right) \;
        2\sqrt{1-\rho}}.
\end{displaymath}
To infer $\theta$ we request $(U, \alpha)$ saying that
$\Prob(\rho > U) = \alpha$, which is given implicitly by
\begin{displaymath}
    \frac{1-\exp\left(-\theta\sqrt{1-U}\right)}{%%
        1-\exp\left(-\sqrt{2}\theta\right)}
    = \alpha
\end{displaymath}
provided that $\alpha$ is larger than the lower limit
$\sqrt{(1-U)/2}$.  We can now take the limit as $\rho_0\rightarrow 1$
which involves the full expression for $C$, and as it turns out that
the solution is the same.


\subsection{The \PCP\ for Toeplitz correlation
    matrices}\label{appendix:toeplitz}

A related problem to computing the \PCP\ for a correlation matrix is
to compute the \PCP\ for the coefficients of an AR$(q)$ process,
\begin{equation}\label{corr:eq1}%
    x_t = \psi_1 x_{t-1} + \cdots + \psi_q x_{t-q} + \epsilon_t,
    \qquad \epsilon_t \;\stackrel{\text{iid}}{\sim}\; {\mathcal N}(0, \tau).
\end{equation}
The corresponding $q\times q$ correlation matrix $\mm{R}$ is now
Toeplitz~\citep{book56}, $R_{ij} = s_{|i-j|}$ where $s_0=1$.
Although~\eref{corr:eq1} is a natural parameterisation for known
$\mm{\psi}$, it is an awkward parameterisation when these are unknown
since the positive definiteness requirement makes the space of valid
$\mm{\psi}$ extremely complicated for $q > 3$. We can use the
invariance property of the \PCP\ to define the prior for $\mm{\psi}$
implicitly.  The basic idea, which is commonly used when estimating
AR($q$) parameters, is that the partial correlations $\mm{\phi} \in
[-1,1]^{p}$,where $p = q-1$, are a useful, unconstrained set of
parameters for this problem.  Furthermore, there is a smooth bijective
mapping between the partial correlations and the autocorrelations
$\mm{s}$ given by the Levinson-Durbin recursions
\citep{monahan1984note,book2}. The base model, which is no
autocorrelation, is transformed to $\mm{\phi} = \mm{I}_{p\times p}$.
Expressed in terms of the partial correlations, the distance function
is $d(\mm{\phi})^{2} = {-\sum_i \log(1-\phi_i^{2})}$, using that
$|\mm{R}| = \prod (1-\phi_i^{2})$.  Define $\gamma_i =
-\log(1-\phi_i^{2})$, for $i=1,\ldots, p$, and the \PCP\ follows
from the simplex formula in Section 6.1 of Simpson \emph{et al.} (2015)  with $h(a) = \sqrt{a}$ and $n = p$. The \PCP\
for $\mm{\phi}$ follows from a change of variables exercise.

The implied pairwise densities for the AR($4$) parameters computed
from $10\,000$ samples with $\lambda=0.3$ are shown in
\Fig{corr:fig2}~(a). It is clear that the parameter space has a
complicated geometry and that the standard prior, which truncates a
multivariate normal prior onto this space
\citep{chib1993bayes,book118}, is suboptimal.  It is also clear from
the geometry of the parameter space that standard MCMC proposals would
have difficulty traversing $\mm{\phi}$--space, whereas
reparameterisation in terms of partial correlations flattens the space
considerably. Panel~(b) shows the histogram for $\psi_1$ based on
$100\,000$ samples from the same prior. While this marginal is
difficult to interpret on its own, it can be understood precisely in
terms of the principles underlying the \PCP\ framework.


\begin{figure}[tbp]
    \centering \mbox{
        \rotatebox{270}{\includegraphics[width=7cm]{ar4-joint.png}}  %%low resolution png for file size
        \makebox[5mm]{}
        \rotatebox{270}{\includegraphics[width=7cm]{ar4-phi1}}}
    \mbox{\makebox[14.5cm]{}} \mbox{%%
        \makebox[7cm]{(a)}%%
        \makebox[5mm]{}%%
        \makebox[7cm]{(b)}}
    \caption{Panel~(a) displays a pairs-plot of $10\,000$ samples from
        the prior for $q=4$ and $\lambda = 0.3$. Panel~(b) shows a
        histogram of the marginal distribution for $\psi_1$ using
        $100\,000$ samples from the same prior.}
    \label{corr:fig2}
\end{figure}



==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU General Public License.
%
% See the files LICENSE_LPPL and LICENSE_GPL for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=0pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

\tikzset{>={triangle 45}}

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}


